PASOA- PArticle baSed Bayesian Optimal Adaptive design

We propose a new procedure named PASOA, for Bayesian experimental design, that performs sequential design optimization by simultaneously providing accurate estimates of successive posterior distributions for parameter inference. The sequential design process is carried out via a contrastive estimation principle, using stochastic optimization and Sequential Monte Carlo (SMC) samplers to maximise the Expected Information Gain (EIG). As larger information gains are obtained for larger distances between successive posterior distributions, this EIG objective may worsen classical SMC performance. To handle this issue, tempering is proposed to have both a large information gain and an accurate SMC sampling, that we show is crucial for performance. This novel combination of stochastic optimization and tempered SMC allows to jointly handle design optimization and parameter inference. We provide a proof that the obtained optimal design estimators benefit from some consistency property. Numerical experiments confirm the potential of the approach, which outperforms other recent existing procedures.

==> pasoa-2/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\hypersetup{
      colorlinks,
      urlcolor={black},
}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage{xcolor}         % colors

\usepackage{subcaption}
\usepackage[most]{tcolorbox}

\usepackage{tikz,pgfplots}
\usetikzlibrary{decorations.text}
\usetikzlibrary{calc}
\newcommand\tikzmark[1]{%
  \tikz[remember picture,overlay]\node (#1) {};%
}

\newcommand\Connect[3][]{%
\tikz[remember picture,overlay]
  \draw[->,red,>=latex,#1] (#2.north east) -- ( $ (#3.north west) + (-20pt,0) $ );%
}
\usetikzlibrary{backgrounds,fit,decorations.pathreplacing, angles, quotes, patterns, math}  % TikZ libraries

%\usepackage{algorithm2e}
%\RestyleAlgo{ruled}


\usepackage{graphicx}
\usepackage{amssymb,amsmath,enumerate}
\graphicspath{{pics/}{figs/}}
\usepackage{afterpage}
\usepackage{textcomp}

%\RequirePackage{amsmath} 
%\RequirePackage{xspace}
\usepackage{xspace}
\usepackage{bbm}

%\usepackage{algorithm} 
%\usepackage{algorithmic}

% DEFINITIONS PRELIMINAIRES
\def\argmax{\mathop{\mathrm{arg\,max}}} % Mieux que \def\argmax{\arg\max}
\def\argmin{\mathop{\mathrm{arg\,min}}} % car l'indice est reparti
%\RequirePackage{amsmath} \RequirePackage{xspace}
%\RequirePackage{bbm}
\usepackage{pifont}
\newcommand{\rcross}{{\color{red}\ding{55}}}
\newcommand{\greencheck}{{\color{green}\checkmark}}


\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}
\def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}
\def\ellb{{\sbm{\ell}}\XS}

% ALPHABET GREC GRAS, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}
\def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}    \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}                 \def\Xib        {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}                 \def\Pib        {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}  \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib       {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib       {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}
\def\upsilonb       {{\sbmm{\upsilon}}\XS}
\def\PM{\kern0pt^{\textrm{{\scriptsize PM}}}\kern0pt}
\def\MMAP{\kern1pt^{\textrm{{\tiny MMAP}}}\kern-1pt}
\def\ML{^{\textrm{{\tiny ML}}}}
\def\dd{\,d}                            % doit etre en italique en anglais
\def\I{\,|\,}           % "sachant" bien espac\'e pour les formules


\newcommand{\w}{\omega}
\newcommand{\g}{\mathcal{G}}
\newcommand{\scalarprod}[2]{{{\bf \langle} {#1},{#2} {\bf \rangle}}}

\newcommand{\Hcondtheta}{H_{\theta\vert Y, T, S}} % loi conditionnelle
\newcommand{\HcondS}{H_{T \vert  S, Y, \theta}} % loi conditionnelle
\newcommand{\HcondT}{H_{S \vert T, Y, \theta}} % loi conditionnelle
\newcommand{\pjcomp}{p_{(Y,S,T)}} %  vraisemblance jointe complete.
\newcommand{\pjcondS}{p_{T \vert S, Y}} % loi conditionnelle
\newcommand{\pjcondT}{p_{S \vert T, Y}} % loi conditionnelle
\newcommand{\pjattach}{p_{Y \vert T, S}} % loi attache donnees
\newcommand{\pjpost}{p_{T, S \vert Y}} % loi a posteriori
\newcommand{\prior}{p_{Z}} % Loi a priori.
\newcommand{\pcomp}{p_{(Y,Z)}} %  vraisemblance complete.
\newcommand{\ppost}{p_{Z \vert Y}} % loi a posteriori
\newcommand{\pattach}{p_{Y \vert Z}} % loi a posteriori
\newcommand{\pinc}{p_{Y}} %  vraisemblance incomplete.
\newcommand{\KL}{\mathrm{KL}} % Distance de Kullback-Leibler
\newcommand{\Nv}{\mathcal{N}} %  voisinage
\newcommand{\DZe}{\mathcal{D}} % Ensemble des probabilites sur Z
\newcommand{\Ind}{\mathcal{I}} % Ensemble des probabilites independantes sur Z
\newcommand{\IndR}{\mathcal{I}_r} % Ensemble des probabilites independantes sur Z + restrictions
%% espaces de probabilites
\def\Prob{\mathbb{P}} % probabilite sur l'espace de la chaine
\def\Exp{\mathbb{E}} % esperance sur l'espace de la chaine
\def\BarExp{\bar{\mathbb{E}}} % esperance sur l'espace  de l'algo
\def\pbar{\bar{\mathbb{P}}} % probabilite sur l'espace de l'algo
%% variables al�atoires et realisations
\newcommand{\tv}{\ensuremath{\mathbf{t}}} % Vecteur des var cachees.(obs)
\newcommand{\sv}{\ensuremath{\mathbf{s}}} % Vecteur des var cachees.(obs)
\newcommand{\Tv}{\ensuremath{\mathbf{T}}} % Vecteur des var cachees.(obs)
\newcommand{\Sv}{\ensuremath{\mathbf{S}}} % Vecteur des var cachees.(obs)
\newcommand{\Wv}{\ensuremath{\mathbf{W}}} % Vecteur des var observees.(obs)
\newcommand{\wv}{\ensuremath{\mathbf{w}}} % Vecteur des var observees.(obs)
\newcommand{\Xv}{\ensuremath{\mathbf{X}}} % Vecteur des var observees.(obs)
\newcommand{\xv}{\ensuremath{\mathbf{x}}} % Vecteur des var observees.(obs)
\newcommand{\Yv}{\ensuremath{\mathbf{Y}}} % Vecteur des var observees.(obs)
\newcommand{\Zv}{\ensuremath{\mathbf{Z}}} % Vecteur des var cachees.(obs)
\newcommand{\yv}{\ensuremath{\mathbf{y}}} % Vecteur des var observees.(obs)
\newcommand{\zv}{\ensuremath{\mathbf{z}}} % Vecteur des var cachees.(obs)
\newcommand{\Ze}{\mathcal{Z}} % Espace d'etat du processus cach\'e.
\newcommand{\B}{{\cal B}}
\newcommand{\taubig}{{\cal T}}
\newcommand{\Be}{\underline{{\cal B}}}
\newcommand{\Phie}{\underline{\Phi}}
\newcommand{\zero}{\ensuremath{\mathbf{0}}}
\def\t{\theta} %parametre
%% Symboles generaux
\def\NNset{\mathbb{N}} % entiers  naturels
\def\Nset{\mathbb{Z}_+} % entiers  naturels
\def\Rset{\mathbb{R}} % reels
%\def\zero{{\mbox{\rm 0\hspace{-0.35em}0}}}  %
\def\un{{\mbox{\rm 1\hspace{-0.25em}I}}}  % indicatrice
\def\ie{\textit{i.e.} } % id est
\def\wp1{\mathrm{w.p.} 1}  % with respect to
\newcommand{\etal}{{\em et al.}} % et al.
%%  GESTION DES DIALOGUES entre AUTEURS
\newenvironment{commentG}
 {\begin{quote}\color{green}\begin{sffamily}}
 {\end{sffamily}\color{black}\end{quote}}
%


\makeatletter

%\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
%\theoremstyle{plain}
\newtheorem{lem}{\protect\lemmaname}
%\theoremstyle{plain}
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{coro}{Corollary}
%\theoremstyle{remark}
\newtheorem{rem}{\protect\remarkname}


\makeatother

\usepackage{babel}
\providecommand{\definitionname}{Definition}
\providecommand{\lemmaname}{Lemma}
\providecommand{\remarkname}{Remark}
\newtheorem{assumption}{{\sf A}\hspace{-3pt}}


%\algrenewcommand\algorithmicindent{0.2em}
